A Layered Aggregate Engine for Analytics Workloads

This paper introduces LMFAO (Layered Multiple Functional Aggregate Optimization), an in-memory optimization and execution engine for batches of aggregates over the input database. The primary motivation for this work stems from the observation that for a variety of analytics over databases, their data-intensive tasks can be decomposed into group-by aggregates over the join of the input database relations. We exemplify the versatility and competitiveness of LMFAO for a handful of widely used analytics: learning ridge linear regression, classification trees, regression trees, and the structure of Bayesian networks using Chow-Liu trees; and data cubes used for exploration in data warehousing. LMFAO consists of several layers of logical and code optimizations that systematically exploit sharing of computation, parallelism, and code specialization. We conducted two types of performance benchmarks. In experiments with four datasets, LMFAO outperforms by several orders of magnitude on one hand, a commercial database system and MonetDB for computing batches of aggregates, and on the other hand, TensorFlow, Scikit, R, and AC/DC for learning a variety of models over databases.

==> aggpush.tex <==
\subsection{Aggregate Pushdown}
\label{sec:aggregate-pushdown}

==> compilation.tex <==
\subsection{Code Compilation}
\label{sec:compilation}

We need to explain:

\begin{itemize}
\item We avoid function calls and recursion.
\item Tuples are structs, generated with exact types. Relations and views are
  dynamic arrays of such tuples. Aggregates are stored as fixed size arrays
  inside structs.
\item Avoid dynamic arrays wherever possible.
\item Order of the aggregates to improve cache locality.
\item Loop unrolling has its limitations, so we use the aggregate register as an
  index to construct very tight loops and avoid blow-up in the number of lines
  we generate
\item We sort the relations once, and views are computed in sorted order, if
  sorted order is not guaranteed during the computation, we append at the end of
  relation and use an index to avoid duplicates, and then sort at end
\begin{itemize}
\item Construct an index that helps to avoid duplicates, we should back this up
  with an example from the code template we generate.
\end{itemize}
\item Parallelization (both task and domain parallelization).
\end{itemize}



==> diagram-macros.tex <==
\tikzstyle{path} = [->,double,rounded corners=.1cm]
\tikzstyle{data} = [draw, rectangle, rounded corners = .07cm, align=center, inner sep = .2cm, outer sep = .1 cm]
\tikzstyle{processor} = [draw, ellipse, align=center, inner sep = .1cm, outer sep = .1 cm]
\colorlet{clr_outofDB}{red!80!black}
\colorlet{clr_inDB}{green!50!black}
\colorlet{clr_inDB_FD}{blue}

\newcommand{\drawtable}[5]
% param#1: width,   param#2: height,   param#3: numCols,   param#4: numRows,   param#5: color
{
   \begin{scope}[shift={(-#1/2,-#2/2)}]
      \pgfmathsetmacro{\cellwidth}{#1/#3}
      \pgfmathsetmacro{\cellheight}{#2/#4}
      \draw[fill=#5!30] (0, #2) rectangle (#1, #2-\cellheight);
      \foreach \i in {1,...,#3}
         \draw[thin, #5!70] (\cellwidth*\i, 0) -- (\cellwidth*\i, #2);
      \foreach \i in {1,...,#4}
         \draw[thin, #5!70] (0, \cellheight*\i) -- (#1, \cellheight*\i);
      \draw[#5] (0, #2-\cellheight) -- (#1, #2-\cellheight);
      \draw[thick, #5] (0, 0) rectangle (#1, #2);
   \end{scope}
}

\newcommand{\drawcylinder}[4]
% param#1: width,   param#2: height,   param#3: top radius,   param#4: color
{
   \begin{scope}[shift={(0,#3/2)}]
      \draw[#4] (0, #2/2) ellipse (#1/2 and #3);
      \draw[#4] (#1/2, -#2/2) arc (0:-180:#1/2 and #3);
      \draw[#4] (-#1/2, #2/2) -- (-#1/2, -#2/2);
      \draw[#4] (#1/2, #2/2) -- (#1/2, -#2/2);
   \end{scope}
}

\newcommand{\drawfilter}[2]
% param#1: width,   param#2: color
{
   \begin{scope}[scale=#1/7, shift={(-3.5,3)}]
      \draw[#2] (0,0)--(7, 0)--(4, -3)--(4,-5)--(3,-6)--(3,-3)--cycle;
   \end{scope}
}

\newcommand*{\highlight}[1]{%
   \tikz\node[rectangle, fill=yellow, inner sep=0.5mm]{#1};%
}


==> parallelism.tex <==
\subsection{Parallelism}
\label{sec:parallelism}


==> problem.tex <==
\section{Problem Statement}
\label{sec:problem}

\mjs{Use $\omega_{R_1}$ as schema for relation $R_1$ to make it consistent with the notation in Section 4.}

We are given a database of $m$ relations $R_1,\ldots,R_m$ over relation schemas $\omega_1,\ldots,\omega_m$. The database schema is $\mathbf{X}=\bigcup_{r\in[m]}\omega_r$. We would like to compute a set of group-by aggregates over the natural join of these relations. This join may represent the training dataset for machine learning models, the input for multi-dimensional data cubes, or the joint probability distribution to be approximated by a Bayesian network. As shown in Section~\ref{sec:applications}, these applications need to compute many queries $Q_i$ of the following form:
\begin{align*}
&\texttt{SELECT } F_i, \texttt{ SUM}(\alpha_{i_1}), \ldots, \texttt{ SUM}(\alpha_{i_n})\\
&\texttt{FROM } R_1 \texttt{ NATURAL JOIN } \ldots \texttt{ NATURAL JOIN } R_m\\
&\texttt{GROUP BY } F_i
\end{align*}
Different queries may have different group-by attributes and aggregates. The user-defined aggregate functions (UDAFs) $\alpha_{i_1},\ldots,\alpha_{i_n}$ can be sums of products of arbitrary functions $f_{ijk}$ over attributes $\omega_{ijk}\subseteq \mathbf{X}$:
\begin{align*}
\alpha_{i_j} = \sum_{j \in [s_i]} \prod_{k\in [p_{ij}]} f_{ijk}(\omega_{ijk}), \mbox{ where } s_i, p_{ij}\in\mathbb{N}
\end{align*}

Section~\ref{sec:applications} gives several examples of UDAFs $f_{ijk}$: it is common for them to be the identity, i.e., returning the parameter attribute, or constants, e.g., 1 for counting. One special case is that of unary UDAFs encoding selection conditions of the form $X_j\text{ op } t$ used for decision trees, where $X_j$ is an attribute, $\text{op}$ is a binary operator, and $t$ is a value in the domain of $X_j$. They can be encoded using the Kronecker delta $\mathbf{1}_{X_j\text{ op } t}$, which evaluates to 1 if the condition is true and 0 otherwise. This has the same effect as pushing these conditions past the join to the input relations. The fewer attributes these UDAFs depend on, the better LMFAO performance reported in Section~\ref{sec:experiments}. UDAFs over many attributes would benefit relatively less from LMFAO. A typical example of an $n$-ary UDAF is $f(\mv X) = e^{\inner{\vec\theta,\mv X}}$, which is an exponential function depending on all attributes $\mv X$ and a vector of real numbers $\vec\theta$ and occurs in the gradient for logistic regression. 

For succinctness, we use an alternative query notation:
    \begin{align}
      Q_i(F_i; \alpha_{i_1}, \ldots, \alpha_{i_n}) & \text{ += } R_1(\omega_1), \ldots, R_m(\omega_m) 
      \label{eq:query}
    \end{align}
We use semicolon to separate the group-by attributes from the aggregate functions in the head of $Q_i$; we omit the semicolon if there are no group-by attributes or no aggregate functions. We use += to capture the SUM over each aggregate function. In the query body, we make explicit the attributes of each relation for a clearer understanding of the definitions of the aggregate functions. By definition, there is a functional dependency between the group-by attributes  and the aggregate functions: $F_i\rightarrow \alpha_{i_1}, \ldots, \alpha_{i_n}$.

Our queries generalize FAQ-SS~\cite{faq} and MPF (Marginalize a Product Function)~\cite{MPF:2000} by allowing tuples of arbitrary UDAFs. 

